Lowest order stabilization free Virtual Element Method for the 2D Poisson equation

We introduce and analyse the first order Enlarged Enhancement Virtual Element Method (E$^2$VEM) for the Poisson problem. The method allows the definition of bilinear forms that do not require a stabilization term, thanks to the exploitation of higher order polynomial projections that are made computable by suitably enlarging the enhancement (from which comes the prefix of the name E$^2$) property of local virtual spaces. The polynomial degree of local projections is chosen based on the number of vertices of each polygon. We provide a proof of well-posedness and optimal order a priori error estimates. Numerical tests on convex and non-convex polygonal meshes confirm the criterium for well-posedness and the theoretical convergence rates.

==> proofHTPoincare.tex <==
\begin{proof}
  Let $\hat{E}\in\Sigma$. First, we want to prove that $\exists C_\Pi(\hat{E})>0$ such that, for all
  $\hat{v}\in\HT{\hat{E}}$,
  \begin{equation} \label{eq:poincare_l1} \int_{\hat{E}}\abs{\hat{v}-\proj[0]{0}{\hat{E}}\hat{v}}
    d\hat{x} \leq C_\Pi(\hat{E}) \left( \sum_{\hat{\tau}\in\Triang{\hat{E}}}
      \int_{\hat{\tau}}\abs{\nabla \hat{v}} d\hat{x} +\sum_{\hat{e} \in\intEdgesReferenceElement}
      \int_{\hat{e}} \abs{\jmp[\hat{e}]{\hat{v}}} \, d\hat{s}\right) \, ,
  \end{equation}
  where $\abs{\nabla \hat{v}}$ denotes the Euclidean norm of $\nabla \hat{v}$.  In order to simplify
  the notation, let us denote by $\mathcal{D}(\hat{v})$ the right hand side of
  \cref{eq:poincare_l1}, i.e.
  \begin{equation*}
    \mathcal{D}(\hat{v}) =
    \sum_{\hat{\tau}\in\Triang{\hat{E}}}  \int_{\hat{\tau}}\abs{\nabla \hat{v}} d\hat{x}
    +\sum_{\hat{e} \in\intEdgesReferenceElement} \int_{\hat{e}} \abs{\jmp[\hat{e}]{\hat{v}}} d\hat{s} \,.
  \end{equation*}
  By contradiction, suppose
  \begin{equation*}
    \label{eq:absurd}
    \forall C>0,\,\exists \hat{v}\in\HT{\hat{E}}\colon\,
    \norm[{\lebl[1]{\hat{E}}}]{\hat{v}-\proj[0]{0}{\hat{E}}\hat{v}} > C \;\mathcal{D}(\hat{v})
    \,.
  \end{equation*}
  Notice that $\mathcal{D}(\hat{v})$ is a seminorm for all $\hat{v}$ in $\HT{\hat{E}}$.  In this
  proof, we consider $\HT{E}\subset\lebl[1]{\hat{E}}$ endowed with the $\lebl[1]{}$-norm. Then, it
  is possible to define a sequence $\hat{w}_k\in\HT{\hat{E}}$ such that, $\forall k\in\mathbb{N}$,
  \begin{equation*}
    \norm[{\lebl[1]{\hat{E}}}]{\hat{w}_k-\proj[0]{0}{\hat{E}} \hat{w}_k} > k \mathcal{D}(\hat{w}_k),
    \quad \norm[{\lebl[1]{\hat{E}}}]{\hat{w}_k-\proj[0]{0}{\hat{E}} \hat{w}_k}=1 \,,
  \end{equation*}
  which means that
  \begin{equation*}
    \mathcal{D}(\hat{w}_k) < \frac{1}{k} \Rightarrow
    \mathcal{D}(\hat{w}_k) \rightarrow 0    \,.
  \end{equation*}
  If we define $\hat{u}_k = \hat{w}_k- \proj[0]{0}{\hat{E}} \hat{w}_k$, we have, since
  $\proj[0]{0}{\hat{E}} \hat{w}_k$ is constant,
  \begin{equation}
    \label{eq:uk_absurd}
    \mathcal{D}(\hat{u}_k) \leq \mathcal{D}(\hat{w}_k)  \rightarrow 0\,.
  \end{equation}
  Then, applying \cref{eq:uk_absurd} and the fact that $\norm[{\lebl[1]{E}}]{\hat{u}_k}=1$, we can
  affirm that the sequence $\hat{u}_k$ is bounded in $\HT{\hat{E}}$.  Thus, it converges weakly in
  $\HT{\hat{E}}$ to a function $\hat{u}^\star$ up to sub-sequences, i.e.
  \begin{equation*}
    \hat{u}_{k_j} \wconv^{\HT{\hat{E}}}
    \hat{u}^\star \,.
  \end{equation*}
  $\HT{\hat{E}}$ is contained in the space of functions of bounded variations, thus it is compactly
  embedded in $\lebl[1]{\hat{E}}$ (see \cite[Corollary 3.49]{AmbrosioLuigi2000Fobv} ). Then,
  $\hat{u}_{k_j}$ converges to a function $\hat{u}^{\star\star}$ strongly in $\lebl[1]{\hat{E}}$, up
  to sub-sequences, and by uniqueness of the limit we have
  $\hat{u}^{\star\star}=\hat{u}^{\star}$. Let $\hat{u}_{\tilde{k}} = \hat{u}_{k_{j_l}} $ be such
  that
  \begin{equation*}
    \hat{u}_{\tilde{k}} \wconv^{\HT{\hat{E}}} \hat{u}^\star,\quad
    \hat{u}_{\tilde{k}}  \sconv^{{\lebl[1]{\hat{E}}}} \hat{u}^\star \,.
  \end{equation*}
  By \cref{eq:uk_absurd} and the definition of $\mathcal{D}$, $ \mathcal{D}(\hat{u}^\star)=0$, thus
  $\hat{u}^\star$ is constant. Since $\norm[{\lebl[1]{\hat{E}}}]{\hat{u}^\star}=1$ then
  $\hat{u}^\star=\frac{1}{\abs{\hat{E}}}$.  It follows that
  \begin{equation*}
    \hat{w}_{\tilde{k}}- \proj[0]{0}{\hat{E}} \hat{w}_{\tilde{k}} \sconv^{{\lebl[1]{E}}}
    \hat{w}^\star- \proj[0]{0}{\hat{E}} \hat{w}^\star= \frac{1}{\abs{\hat{E}}}
  \end{equation*}
  by continuity and linearity of $\proj[0]{0}{\hat{E}}$.  By definition of $\proj[0]{0}{\hat{E}}$,
  this is a contradiction since
  \begin{equation*}
    \hat{w}^\star-\proj[0]{0}{\hat{E}} \hat{w}^\star = const \imply const = 0 \,,
  \end{equation*}
  then, \cref{eq:poincare_l1} is true.  Next, since $\HT{\hat{E}}$ is continuously embedded in
  $\lebl{\hat{E}}$ (see \cite[Corollary 3.49]{AmbrosioLuigi2000Fobv}), endowing $\HT{\hat{E}}$ with the $\lebl[1]{}$-norm, we have
  \begin{equation}\label{eq:contEmbeddingPoincare}
    \exists C_I(\hat{E}) > 0\colon  \norm[\lebl{\hat{E}}]{\hat{v}-\proj[0]{0}{\hat{E}}\hat{v}} \leq
    C_I(\hat{E}) \norm[{\lebl[1]{\hat{E}}}]{\hat{v}-\proj[0]{0}{\hat{E}}\hat{v}} \,.
  \end{equation}
  Moreover, by H\"older's inequality and since $h_{\hat{E}}=1$, we get, exploiting also Young's
  inequality,
  \begin{equation}\label{eq:holderInPoincare}
    \begin{split}
      \mathcal{D}(\hat{v})^2 &=\left( \sum_{\hat{\tau}\in\Triang{\hat{E}}}
        \int_{\hat{\tau}}\abs{\nabla \hat{v}} d\hat{x} +\sum_{\hat{e} \in\intEdgesReferenceElement}
        \int_{\hat{e}} \abs{\jmp[\hat{e}]{\hat{v}}} d\hat{s} \right)^2
      \\
      &\leq \left( \sum_{\hat{\tau}\in\Triang{\hat{E}}} \left(\int_{\hat{\tau}}
          d\hat{x}\right)^{\frac12} \left( \int_{\hat{\tau}} \abs{\nabla \hat{v}}^2
          d\hat{x}\right)^{\frac12} + \sum_{\hat{e}\in\intEdgesReferenceElement} \left(
          \int_{\hat{e}} d\hat{s} \right)^{\frac12} \left( \int_{\hat{e}} \jmp[\hat{e}]{\hat{v}}^2
          d\hat{s}\right)^{\frac12} \right)^2
      \\
      & \leq 2\NVE \left(\sum_{\hat{\tau}\in\Triang{\hat{E}}} \abs{\hat{\tau}}
        \norm[\lebl{\hat{\tau}}]{\nabla \hat{v}}^2 + \sum_{\hat{e} \in \intEdgesReferenceElement}
        h_{\hat{e}} \norm[\lebl{\hat{e}}]{\jmp[\hat{e}]{\hat{v}}}^2\right) \leq 2 \NVE
      \seminorm[\HT{\hat{E}}]{\hat{v}}^2\,,
    \end{split}
  \end{equation}
  since $\abs{\hat{\tau}} \leq \abs{\hat{E}} \leq h_{\hat{E}}^2=1$ and $h_e \leq h_{\hat{E}} = 1$.
  From \cref{eq:poincare_l1}, \cref{eq:contEmbeddingPoincare} and \cref{eq:holderInPoincare}, we
  obtain that $\exists C(\hat{E}) = \sqrt{2\NVE}C_\Pi(\hat{E})C_I(\hat{E}) > 0$ such that
  \begin{equation} \label{eq:boundPoincareHatE}
    \norm[\lebl{\hat{E}}]{\hat{v}-\proj[0]{0}{\hat{E}}\hat{v}}\leq C(\hat{E})
    \seminorm[\HT{\hat{E}}]{\hat{v}} \,.
  \end{equation}
  We are left to show that there exists a constant independent of $\hat{E}$ for which
  \cref{eq:Poincare HT} holds. This is true because we can divide by $\seminorm[\HT{\hat{E}}]{\hat{v}}$, since the case $\seminorm[\HT{\hat{E}}]{\hat{v}}=0$ is trivial, and obtain the ratio
  \begin{equation*}
    \frac{\norm[\lebl{\hat{E}}]{\hat{v}-\proj[0]{0}{\hat{E}}\hat{v}}}
    {\seminorm[\HT{\hat{E}}]{\hat{v}}} \,,
  \end{equation*}
  which is a continuous function with respect to $\hat{E}$ and also bounded by
  \cref{eq:boundPoincareHatE}. Thus, since $\Sigma$ is a compact set by
  \cref{lem:compactnessSigma}, then there exists
  $\hat{E}^\star \in\Sigma$ such that, $\forall \hat{E}\in \Sigma$,
  \begin{equation*}
    \norm[\lebl{\hat{E}}]{\hat{v}-\proj[0]{0}{\hat{E}}\hat{v}}\leq C(\hat{E}^\star)
    \seminorm[\HT{\hat{E}}]{\hat{v}} \,,
  \end{equation*}
  thus proving \cref{eq:Poincare HT} with $C=C(\hat{E}^\star)$.
\end{proof}
